Motivic nearby cycles functors, local monodromy and universal local acyclicity

In this thesis we give two applications of Ayoub's motivic nearby cycles functor: First we give a generalization of Grothendieck's classical local monodromy theorem. In the classical setup we show that the inertia group acts quasi-unipotently on the \'etale cohomology of sheaves 'coming from motives'. Second we study the notion of universal local acyclicity for motives and show that for \'etale motives universal local acyclicity over an excellent 1- dimensional regular base scheme is detected by the motivic nearby cycles functor. Along the way we prove properties of the motivic nearby cycles functor which might be of independent interest. In particular we show that with rational coefficients the unipotent motivic nearby cycles functor is a direct summand of the total motivic nearby cycles functor.

==> ChapterLog.tex <==
\chapter{The Log-Motive and the Unipotent Nearby Cycles Functor}

\section{The Universal Property of the Log-Motive}

\noname \label{noname:SimplObjAssToSpan} Let $\C$ be a 1-category with finite products and consider a span
\[
A \overset{f}\longrightarrow B \overset{g}\longleftarrow C
\]
in $\C$. Then as in \cite[3.4.1]{AyoubThesisII} we can associate to this span a co-simplicial object
\[
A \tilde{\times}_B C: \Delta \longrightarrow \C
\]
with
\[
A \tilde{\times}_B C(i) = A \times B^{i} \times C
\]
for $i$ in $\Delta$ and co-face and co-degeneracy maps given by:
\begin{enumerate}
\item $d_0: (a, b_0,\dots, b_i, c) \mapsto (a, f(a), b_0,\dots, b_i, c)$.
\item $d_k: a, b_0,\dots, b_i, c) \mapsto a, b_0,\dots, b_k, b_k, \dots b_i, c)$ for $0<k<i$.
\item $d_i: (a, b_0,\dots, b_i, c) \mapsto (a, b_0,\dots, b_i, g(c), c)$.
\item $s_k:(a, b_0,\dots, b_i, c) \mapsto (a, b_0,\dots, \widehat{b_k}, \dots, b_i, c)$ for $0 \leq k \leq i$.
\end{enumerate}
Let us denote the category of spans in $\C$ by $\C^{\rightarrow \leftarrow}$. It is easy to see that this construction gives rise to a functor
\[
\bullet \tilde{\times}_{\bullet} \bullet : \C^{\rightarrow \leftarrow} \longrightarrow \Fun (\Delta , \C). 
\]

\noname Let $S$ be a qcqs scheme and $(X,s)$ a smooth pointed $S$-scheme. By this we mean a smooth scheme $\pi: X \rightarrow S$ over $S$ together with a section $s: S \rightarrow X$ of $\pi$. Consider the span
\[
[X \overset{\id}\rightarrow X] \overset{\Delta}\longrightarrow [X \times_S X \overset{p_1}\rightarrow X] \overset{(\id, s)}\longleftarrow [X \overset{\id}\rightarrow X]
\] 
in $\Sm_{/X}$. As above we can associate to such a span a co-simplicial object
\[
\mathcal{A}_{(X,s)}: \Delta \longrightarrow \Sm_{/X}
\]
with
\[
\mathcal{A}_{(X,s)}(i) = [X \times_S X^{\times i} \overset{p_1}\rightarrow X]
\]
for $i$ in $\Delta$.


Via the functor
\[
\Sigma^\infty: \Sm_X \longrightarrow \SH(X)
\]
as for example considered in \cite[2.39]{Robalo15} the co-simplicial scheme $\mathcal{A}_{(X,s)}$ gives rise to a co-simplicial object
\[
\Log_{(X,s)}: \Delta \overset{\mathcal{A}_{(X,S)}}\longrightarrow \Sm_{/X} \overset{\Sigma^\infty}\longrightarrow \SH(X).
\]
 Let $\T(\_)$ be a six-functor formalism over $S$. By this we mean a $(*,\#, \otimes)$-formalism on $(\Sch^{\qcqs}_{/S}, \Sm_{/S})$ satisfying the Voevodsky-conditions in the sense of \cite{Adeel6Functor}. Then there exists a unique system of colimit preserving functors
\[
R_Y: \SH(Y) \longrightarrow \T(Y)
\]
for all $Y$ in $\Sch^{\qcqs}_{/S}$ which commute with $f^*$ , tensor-product and $f_\#$ for smooth $f$ (see \cite[2.14]{Adeel6Functor}). We denote the co-simplicial object
\[
\Delta \overset{\Log_{(X,s)}}\longrightarrow \SH(X) \overset{R_X}\longrightarrow \T(X)
\]
again by $\Log_{(X,s)}$ and call it the \textit{logarithm motive associated to} $(X,s)$.

The structure of $\mathcal{A}_{(X,s)}$ as a co-simplicial $X$-scheme induces a canonical map
\begin{equation} \label{eqn:EpsilonLog}
\varepsilon: \Log_{(X,s)} \rightarrow \underline\1
\end{equation}
in $\Fun(\Delta,\T(X))$, where $\underline\1$ denotes the constant functor with value $\1$. It is easy to see that the co-simplicial object 
\[s^* \Log_{(X,s)}: \Delta \overset{\Log_{(X,s)}}\longrightarrow \T(X) \overset{s^*}\longrightarrow \T(S)
\]
is equivalent to the co-simplicial object in $\T(S)$ obtained analogously as above from the span
\[
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRGQGUACAHR4howATnBg5gfLFAC+fIVgDmACxx0hQiAHcuHCiGml0mXPkIoAjOSq1GLNsi4ANXv0EixEnmiyye85arqWjp6BkbYeAREAExW1PTMrIjs3HwCwqLikjJyiipqGtq6+tYwUArwRKAAZhoAtkhkIDgQSJY2iWx8ACIwDKr6hiC1EA2Isc2tiO0JdskI1Ax0AEZ9AArGkWYg-iol0kA
\begin{tikzcd}
{[S \overset{\id}\rightarrow S]} \arrow[r, "s"] & {[ X \overset{\pi}\rightarrow S]} & {[S \overset{\id}\rightarrow S]} \arrow[l, "s"']
\end{tikzcd}
\]
in $\Sm_{/S}$. In particular there is a canonical map
\[
\eta:\underline\1  \rightarrow s^*\Log_{(X,s)}
\]
in $\Fun(\Delta,\T(S))$ induced by the map of spans
\[
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBoBGAXVJADcBDAGwFcYkRkBlAAgB1eItGACc4MHMH5YoAX37CsAcwAWOesOEQA7t06UQM0uky58hFOQrU6TVu2TcAGnwFDR4ybzRY5vBSrUNbV19Q2NsPAIiACYrGgYWNkQOHn5BETEJKVl5JVV1TR09AyMQDAizIktiawS7ZK4XdPcs3mlff3ygotDS8tMolDIa+NsklKa3TM923ICC4OKwspNI82RYkZtE+1TXDI9sjrzAwpCDaxgoRXgiUAAzTQBbJDIQHAgkS236kARlx4QF6IWLvT6Ib51cYIGiMegAIxgjAACqtKslOjgSg9nkgAKw0D5IUFwxEotGDECYkCjHbJbLYkCA4EAZkJ4MhY3Y-1KzKQABZ2a9ab8GQDcYhBWCkGyfuMxbyJQTpYhZVD2AzYQikaiKpTqTJKDIgA
\begin{tikzcd}
{[S \overset{\id}\rightarrow S]} \arrow[d, "\id"] \arrow[r, "\id"] & {[S \overset{\id}\rightarrow S]} \arrow[d, "s"] & {[S \overset{\id}\rightarrow S]} \arrow[d, "\id"'] \arrow[l, "\id"'] \\
{[S \overset{\id}\rightarrow S]} \arrow[r, "s"]                    & {[ X \overset{\pi}\rightarrow S]}               & {[S \overset{\id}\rightarrow S]} \arrow[l, "s"']                    
\end{tikzcd}
\]
in $\Sch^{\qcqs}_{/S}$.

\begin{lem} \label{lem:CompEtas^*EpsilonIsID}
Let $(\pi:X \rightarrow S,s)$ be a smooth pointed $S$-scheme. Then the composition
\[
\underline\1 \overset{\eta}\longrightarrow s^*\Log_{(X,s)} \overset{s^* \varepsilon}\longrightarrow \underline\1
\]
is equivalent to the identity. 
\end{lem}

\begin{proof}
This follows from the fact that this composition is induced by the top to bottom composition of spans
\[
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBoBGAXVJADcBDAGwFcYkRkBlAAgB1eItGACc4MHMH5YoAX37CsAcwAWOesOEQA7t06UQM0uky58hFOQrU6TVu2TcAGnwFDR4ybzRY5vBSrUNbV19Q2NsPAIiACYrGgYWNkQOHn5BETEJKVl5JVV1TR09AyMQDAizIktiawS7ZK4XdPcs3mlff3ygotDS8tMolDIa+NsklKa3TM923ICC4OKwspNI82RYkZtE+1TXDI9sjrzAwpCS8IH1smjasd3Jg9bZvxOFnouVisHkS1vRnYNPbNaZHOZdM5LPqrSooWL-bb1CZpKaHNo5V7zbrnGTWGBQRTwIigABmmgAtkgyCAcBAkJZEeMEMsyRBKYhYjS6YgGXUmSAaIx6AAjGCMAAKMMGIE6OE+rPZAFYaLSkJyhaKJVLzCBGDASXKAUjsvKKUgAMwq7m8+7JZmlBVIAAsVqpRvGJpZZsQLq5Fvd7E9Du9yr9iEtjMD6IFupFYsl3x1stNbLVrsQAA4A8kg6TvVmwwB2bMgE2CuNaxPsZNe1OIABs6eLkZz0dr7OpqobJdzIEdPKbPa8WAMlBkQA
\begin{tikzcd}
{[S \overset{\id}\rightarrow S]} \arrow[d, "\id"] \arrow[r, "\id"] & {[S \overset{\id}\rightarrow S]} \arrow[d, "s"]    & {[S \overset{\id}\rightarrow S]} \arrow[d, "\id"] \arrow[l, "\id"'] \\
{[S \overset{\id}\rightarrow S]} \arrow[r, "s"] \arrow[d, "\id"]   & {[ X \overset{\pi}\rightarrow S]} \arrow[d, "\pi"] & {[S \overset{\id}\rightarrow S]} \arrow[l, "s"'] \arrow[d, "\id"]   \\
{[S \overset{\id}\rightarrow S]} \arrow[r, "\id"]                  & {[S \overset{\id}\rightarrow S]}                   & {[S \overset{\id}\rightarrow S]} \arrow[l, "\id"']                 
\end{tikzcd}
\]
which is the identity. 


\end{proof}


\begin{definition} Let $\pi: X \rightarrow S$ a smooth map and $\T(\_)$ a six functor formalism. We denote the smallest stable full subcategory of $\T(X)$ containing the objects of the form $\pi^*A$ for all $A$ in $\T(S)$ by $\Uni_\pi(X)$. An object $M$ in $\Uni_\pi(X)$ is called \textit{unipotent}.
\end{definition}

\begin{remark} For a smooth pointed $S-$scheme $(X,s)$ we have 
\[ \Sigma^\infty \mathcal{A}_{(X,s)}(i) \simeq [X \times_S X^{\times i} \overset{p_1}\rightarrow X] \simeq \pi^* \Sigma^\infty [X^{\times i} \rightarrow S]. 
\]
Hence $\Log_{(X,s)}$ factors as
\[
\Log_{(X,s)}: \Delta \longrightarrow \Uni_\pi(X) \subset \T(X).
\]
\end{remark}



\begin{lem} \label{lem:GenOfAyoubsThm}
Let $(\pi:X \rightarrow S,s)$ be a smooth pointed $S$- scheme. Then for any $A$ in $\T(S)$ the composition
\[
A \overset{\unit}\longrightarrow \pi_* \pi^* A \overset{\varepsilon^\#}\longrightarrow \colim_{\Delta^{op}}\pi_*\Hom(\Log_{(X,s)},\pi^* A ),
\]
where the last arrow is induced by precomposition with (\ref{eqn:EpsilonLog}), is an equivalence.
\end{lem}

\begin{proof}
Using the notations of ?? let us consider the maps $(\theta, \id_\Delta) :(\mathcal{A}_{(X,s)}, \Delta) \rightarrow (X,\Delta)$, $(\pi, \id_\Delta): (X, \Delta) \rightarrow (S, \Delta)$ and $p_\Delta: (S,\Delta) \rightarrow (S, \star)$. Then by ?? the assertion of the Lemma is equivalent to saying that the composition
\begin{align*}
A &\longrightarrow \pi_* \pi^* A \\
&\overset{\sim}\longrightarrow (p_\Delta)_\# (\pi, \id_\Delta)_*(\pi, \id_\Delta)^* (p_\Delta)^* A \\
&\longrightarrow (p_\Delta)_\# (\pi, \id_\Delta)_*(\theta, \id_{\Delta})_*(\theta, \id_{\Delta})^*(\pi, \id_\Delta)^* (p_\Delta)^* A
\end{align*}
is an equivalence. This can be shown analogous to \cite[3.4.9]{AyoubThesisII}: Note that the co-simplicial $S$-scheme obtained by considering $\mathcal{A}_{(X,s)}$ as an $S$-scheme via $\pi:X \rightarrow S$ is equivalent to the co-simplicial scheme obtained by applying the construction of ?? to the span
\[
[X \overset{\pi}\rightarrow S] \overset{\id}\longleftarrow [X \overset{\pi}\rightarrow S] \overset{s}\longleftarrow [S \overset{\id}\rightarrow S].
\]
In particular the canonical map 
\end{proof}


\noname \label{noname:CanMapForUnivPropOfLog} For any $M$ in $\T(X)$ there is a cnaonical comparison map 
\begin{align*}
\pi_* \Hom(\Log_{(X,s)}, M) & \overset{\unit}\longrightarrow \pi_* s_* s^* \Hom(\Log_{(X,s)}, M) \\
& \overset{\sim}\longrightarrow s^* \Hom(\Log_{(X,s)}, M) \\
& \longrightarrow  \Hom(s^*\Log_{(X,s)}, s^* M) \\
& \overset{\eta^\#}\longrightarrow s^* M,
\end{align*}
where the last arrow is induced by $\eta:\1  \rightarrow s^*\Log_{(X,s)}$. 


\begin{thm} Let $(\pi:X \rightarrow S,s)$ be a smooth pointed $S$- scheme. Then for any $M$ in $\Uni(X)$ the comparison map
\[
\pi_* \Hom(\Log_{(X,s)}, M) \longrightarrow s^* M
\]
of \ref{noname:CanMapForUnivPropOfLog} is an equivalence.
\end{thm}

\begin{proof}
It suffices to show the claim for $M = \pi^*A$ and $A$ in $\T(S)$. Consider the following diagram:
\[
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRAEEQBfU9TXfIRQBGclVqMWbADrS0WAPoAqWfIB6Szjz7Y8BIgCYx1es1aIQqxSukAJCAFsAFLIAyEAOYLgTgBqk4AEoeAAIrDXZA7l4QDF1BQ1JhcVMpCytlOGUQuA1Ze2c3T28-AODSMLksCKjtWP49IWQjAxTJcxAcvLtHF2l3Lx9-INDwzVqYuIF9FCMAZjazGR7nLpsBkuHykLWxyOidaaajABZFtM7cpUr1a61JhoSRJPOOjKUs66u9g-r4meQolaJnabCuN2qd1+U0aRFECxBSws4LGIS04hgUA88CIoAAZgAnRxIMggHAQJCiCRIyzSJhgXC-QnExCk8lIADsiIusmwDhA1AYdAARjAGAAFR4zEAErAeAAWOCZRP5iCp7MQXOpPLpDKVdWZqvVFMQRm1b2k9AJMDQ2AY+gNKs51A1c25FqtNrtDpihqQZtd7uW9MZjpZWo1AA4g+lpHyBSAhaKJVKhDK5YrlSy3WSTScY7T42HVdHc0gTsWkKWNQBOAuyLBQBNJsWS-5p2UK-W+p2IfNlxAAVkriDrA8HBe+lro1ttWHthBHY41ADZ69JG82Ra3U2xO5mRxOB2vzcsYDg6FnVf3a4Ltyn22wsGBsLAE6kOk5hLUKFwgA
\begin{tikzcd}
A \arrow[r, "\unit"] \arrow[rd, "\sim"'] & \pi_*\pi^*A \arrow[d, "\unit"] \arrow[r, "\varepsilon^\#"]        & {\pi_*\Hom(\Log_{(X,s)}, \pi^*A)} \arrow[d, "\unit"]                     \\
                                         & \pi_*s_* s^*\pi^*A \arrow[r, "\varepsilon^\#"] \arrow[d, "\sim"'] & {\pi_*s_* s^*\Hom(\Log_{(X,s)}, \pi^*A)} \arrow[d, "\sim"]               \\
                                         & s^* \pi^* A \arrow[r, "\varepsilon^\#"] \arrow[d, "\id"']                        & { s^*\Hom(\Log_{(X,s)}, \pi^*A)} \arrow[d] \arrow[ld, "(1)" description, phantom] \\
                                         & s^* \pi^* A \arrow[r, "(s^*\varepsilon)^\#"] \arrow[rd, "\id"']     & {\Hom( s^*\Log_{(X,s)},  s^*\pi^*A)} \arrow[d, "\eta^\#"]                   \\
                                         &                                                                &  s^* \pi^* A.                                                            
\end{tikzcd}
\]
Here the supscript $(\_)^\#$ denotes precomposition with the respective map. The composition of the top horizontal row is an equivalence by Lemma \ref{lem:GenOfAyoubsThm} and the right vertical composition is the comparison map of \ref{noname:CanMapForUnivPropOfLog}. Hence it remains to show that the diagram commutes. The commutativity of the bottom triangle follows from Lemma \ref{lem:CompEtas^*EpsilonIsID} and commutativity of the unmarked squares is obvious. The transposed diagram of $(1)$ with respect to the $\otimes \dashv \Hom$ adjunction is
\[
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRDgD0AqAAgB0+aLNx4BZfnwh4AtvB6deAgDIQA5gH1gACgAapOAEoAviCOl0mXPkIoAjOSq1GLNgokAJCNK3K1m3frGAkIiogYSUliycPIivhraeoYmZhbYeARE9raO9MysiOxxgsK8oqaOMFCq8ESgAGYATl5I9iA4EEgATNR5LoVuAjA0puYgTS2IZO2diD1O+WxaCgL0jTBo2AwEBhwCAMQg1Ax0AEYwDAAKlhk2II1YqgAWOKMNzdJI0x2tvc4FIFWdHWmyw2zAez4+wiMngAiwUAqRiAA
\begin{tikzcd}
{s^* \pi^* A \otimes s^* \Log_{(X,s)}} \arrow[rd, "\id \otimes (s^*\varepsilon)^\#"'] \arrow[r, "\varepsilon^\# \otimes\id"] & {s^* \Hom(\Log_{(X,s)}\pi^* A) \otimes s^* \Log_{(X,s)}} \arrow[d, "s^* \ev"] \\
                                                                                                                 & s^* \pi^* A                                                                  
\end{tikzcd}
\] 
which obviously commutes.
\end{proof}

\begin{cor}
$\Log$ is a pro-object. 
\end{cor}

\begin{cor}
Assume that $\T$ is $\DA_{\et}( \_, \Lambda)$, where $\Lambda$ is a $\Q$-algebra. Let $X$ be a smooth group scheme over $S$ and $s: S \rightarrow X$ the unit section. If either $S$ is of characteristic $0$ or $X$ is affine then $\Log_{(X,s)}$ coincides with the logarithm motive defined in [HK].
\end{cor}

\begin{cor}
Adjunction. 
\end{cor}

\begin{cor}
Realizations of Log.
\end{cor}

\begin{prop}

Let $f: (X,x) \rightarrow (Y,y)$ be a morphism of smooth pointed $S$-schemes. Then there exists a unique map $\gamma_f: \Log_{(X,x)} \rightarrow f^* \Log_{(Y,y)}$ in $\Pro \T(X)$ 
with the property that 
\[
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZARgBoAGAXVJADcBDAGwFcYkQAdD4kAX1PSZc+QinKli1Ok1bsAHgD0AVAAIuAGQgBzAPrAAFAA1ScgJS8+AkBmx4CRMpJoMWbRCEWqAZsrUdNugYAmqQAnuaWgrYiRABMElIusu6hyhraevoh4Ra8UjBQWvBEoF4AThAAtkhkIDgQSPHSrvK+XFr0lZX0Ol6RIOVVSOJ1DYi1SW6cHDA4PQbGZhY0jPQARjCMAApCdqIgZVhaABY4-YPViCP1SADMzjJTXLPzWWER-KUVl003iPcgY4wehQdiQMBsB4tdxcbDVPK8IA
\begin{tikzcd}
                                             & \1 \arrow[ld, "{\eta_{(X,x)}}"'] \arrow[rd, "{\eta_{(Y,y)}}"] &                   \\
{x^* \Log_{(X,x)}} \arrow[r, "x^* \gamma_f"] & {x^* f^* \Log_{(Y,y)}} \arrow[r, "\sim", no head]             & {y^*\Log_{(Y,y)}}
\end{tikzcd}
\]
commutes. 

\end{prop}


\section{The Log Motive of $\G_m$ and Nearby Cycles}

\begin{remark}
Coincides with Ayoubs Log.
\end{remark}

\begin{thm}
Let $(X,s)$ be a smooth pointed $S$-scheme. Then there is a fiber sequence
\[
\Log_{(X,s)}(1) \overset{N}\longrightarrow \Log_{(X,s)} \overset{\varepsilon}\longrightarrow \1
\]
in $\Pro (\Uni(X)).$
\end{thm}

\begin{cor}
Kummer motive in SH
\end{cor}


\noname Intro of $\Upsilon$. And monodromy sequence. 

\begin{prop} Let $f:X \rightarrow S$ be of finite type and $M$ a constructible object of $\T(X_\eta)$. Then $\Upsilon_f(M)$ is constructible.
\end{prop}

\begin{proof}
...
\end{proof}

\section{Application: Euler-Charactersitics vs. Euler-Characteristics with compact support}

\begin{thm}
$f_! = f_*$ in $K/(\1- \1(1))$.
\end{thm}


\begin{cor}
Euler characteristics etc.
\end{cor}

